Learning Successive Interference Cancellation for Low-Complexity Soft-Output MIMO Detection

Low-complexity multiple-input multiple-output (MIMO) detection remains a key challenge in modern wireless systems, particularly for 5G reduced capability (RedCap) and internet-of-things (IoT) devices. In this context, the growing interest in deploying machine learning on edge devices must be balanced against stringent constraints on computational complexity and memory while supporting high-order modulation. Beyond accurate hard detection, reliable soft information is equally critical, as modern receivers rely on soft-input channel decoding, imposing additional requirements on the detector design. In this work, we propose recurSIC, a lightweight learning-based MIMO detection framework that is structurally inspired by successive interference cancellation (SIC) and incorporates learned processing stages. It generates reliable soft information via multi-path hypothesis tracking with a tunable complexity parameter while requiring only a single forward pass and a minimal parameter count. Numerical results in realistic wireless scenarios show that recurSIC achieves strong hard- and soft-detection performance at very low complexity, making it well suited for edge-constrained MIMO receivers.

==> befe.tex <==
\usepackage{mathtools}	% loads amsmath
\usepackage{amssymb}
\usepackage{amsthm}

\usepackage[utf8]{inputenc}

\usepackage{ifthen}

% char­ac­ter pro­tru­sion and font ex­pan­sion, fur­ther­more the ad­just­ment of in­ter­word
% spac­ing and ad­di­tional kern­ing, as well as hy­phen­at­able let­terspac­ing (track­ing)
% and the pos­si­bil­ity to dis­able all or se­lected lig­a­tures.
\usepackage{microtype}

% customizing captions in floating environments
%\usepackage{caption}

% bold letters
\usepackage{bm}

\RequirePackage{algorithm}
\RequirePackage{algorithmic}

\usepackage{siunitx} % for SI units and more, see https://texdoc.org/serve/siunitx/0

\usepackage[draft,nomargin,marginclue,inline]{fixme}
% draft mode: creates no compilation aborts, final mode does
% nomargin: do not show note in margin
% marginclue: indicate in margin that there is a note
% inline: display note inline
\renewcommand*\FXLayoutInline[3]{{[\textcolor{red}{{#2}}]}}	% make inline note red
\makeatletter
\renewcommand*\FXLayoutMarginClue[3]{%
	\marginpar[%
	\raggedleft\@fxuseface{margin}\textcolor{red}{\ignorespaces $ \Rightarrow $}]{%
		\raggedright\@fxuseface{margin}\textcolor{red}{\ignorespaces $ \Leftarrow $}}}
\makeatother	% change color and displayed text in margin
% for twocolumn: increase width of margin notes - this fixes problem with left \fixme
%\setlength{\marginparwidth}{24pt}

\usepackage{tumcolor}

\usepackage{pgfplotstable}	% loads pgfplots, tikz
% tikz loads xcolor, graphicx, ...

% to load CSV data
% use: 	discard if={<column name>}{<value>}
%		discard if not={<column name>}{<value>}
\pgfplotsset{
	discard if/.style 2 args={
		x filter/.append code={
			\edef\tempa{\thisrow{#1}}
			\edef\tempb{#2}
			\ifx\tempa\tempb
			\def\pgfmathresult{inf}
			\fi
		}
	},
	discard if not/.style 2 args={
		x filter/.append code={
			\edef\tempa{\thisrow{#1}}
			\edef\tempb{#2}
			\ifx\tempa\tempb
			\else
			\def\pgfmathresult{inf}
			\fi
		}
	}
}

\usepackage{cite}

% \usepackage{hyperref}
% % some of these options need the package xcolor
% \hypersetup{
% 	colorlinks = true,
% 	% border around links like \eqref
% 	linkbordercolor = {white},
% 	% color of numbers in \cite
% 	citecolor = {black},
% 	% color of letters in links like \eqref
% 	linkcolor = {black},
% 	% color of letters in url
% 	urlcolor = {black}
% }
% starred ref environment
% \makeatletter
% \renewcommand*{\eqref}[1]{%
% 	\hyperref[{#1}]{\textup{\tagform@{\ref*{#1}}}}%
% }
% \makeatother

% intelligent cross-referencing
\usepackage{cleveref}

% supports acronyms and multiple glossaries
% use \acp for plural
\usepackage[acronym,shortcuts]{glossaries}


\pgfplotsset{
  % ---------------------------
  % Baselines (more "classic")
  % ---------------------------
  sd/.style={
    color=gray,
    mark=o,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  mmse/.style={
    color=TUMBeamerOrange,
    mark=triangle,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
    % dashdotted,
  },
  mmse-vblast/.style={
    color=TUMBeamerRed,
    mark=star,
    dashed,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  zf-vblast/.style={
    color=brown,
    dotted,
    mark=x,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  % ----------------------------------------
  % recurSIC family (consistent "own" theme)
  % ----------------------------------------
  % Use stronger colors + dash patterns to be distinct as a group.
  recurSIC-K1/.style={
    color=TUMLightBlue,
    solid,
    mark=diamond,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  recurSIC-K2/.style={
    color=TUMLighterBlue,
    dashed,
    mark=diamond,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  recurSIC-K4/.style={
    color=TUMBeamerBlue,
    dashdotted,
    mark=diamond,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  recurSIC-K6/.style={
    color=TUMBlueDarker,
    densely dashed,
    mark=diamond,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  recurSIC-K8/.style={
    color=blue,
    densely dashdotted,
    mark=diamond,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
  recurSIC-K10/.style={
    color=violet,
    densely dotted,
    mark=diamond,
    mark options={solid},
    line width=\lineWidth,
    mark size=\marksize,
  },
}


%new commands
\newcommand{\op}[1]{{\operatorname{#1}}}
\newcommand{\uproman}[1]{\uppercase\expandafter{\romannumeral#1}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\del}{_{\bm{\delta}}}
\newcommand{\deli}{_{\bm{\delta}_i}}
\newcommand{\eye}{\bm{\op{I}}}
\newcommand{\B}[1]{\bm{#1}}
\newcommand{\inv}{^{-1}}
\newcommand{\invt}{^{-\frac{1}{2}}}
\newcommand{\h}{^{\op H}}
\newcommand{\T}{^{\op T}}
\newcommand{\siginv}{\frac{1}{\sigma^2}}
\newcommand{\xfac}{\sum_{i=1}^{N}|x_i|^2}
\newcommand{\Chat}{\widehat{\B C}}
\newcommand{\chat}{\hat{\B c}}
\newcommand{\sqrtinv}{\frac{1}{\sqrt{2}}}
\newcommand{\NC}{\mathcal{N}_{\C}}
\newcommand{\hhat}{\hat{\B h}}
\newcommand{\E}{\mathbb{E}}
\DeclareMathOperator{\dft}{\mathbf{F}}




\tikzset{genie_em/.style={mark options={solid},color=black, line width=\lineWidth, mark size=\marksize}}
\tikzset{genie_blmmse/.style={mark options={solid},color=darkgray, line width=\lineWidth, mark size=\marksize,dashed}}
\tikzset{global_em/.style={mark options={solid},color=TUMBeamerRed, line width=\lineWidth, mark=diamond, mark size=\marksize,dashdotted}}
\tikzset{global_blmmse/.style={mark options={solid},color=TUMOrange, line width=\lineWidth, mark=triangle, mark size=\marksize,dashdotted}}
\tikzset{gmm2/.style={mark options={solid},color=teal, line width=\lineWidth, mark=square, mark size=\marksize,dashed}}
\tikzset{gmm3/.style={mark options={solid},color=violet, line width=\lineWidth, mark=pentagon, mark size=\marksize,dashed}}
\tikzset{gmm/.style={mark options={solid},color=TUMBeamerBlue, line width=\lineWidth, mark=o, mark size=\marksize}}
\tikzset{em_gm_gamp/.style={mark options={solid},color=magenta, line width=\lineWidth, mark=x, mark size=\marksize,dotted}}
\tikzset{gmm_blmmse/.style={mark options={solid},color=brown, line width=\lineWidth, mark=|, mark size=\marksize,dotted}}

% math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\expec}{E}
\DeclareMathOperator{\lin}{span}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\supp}{supp}
%\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\uvect}{vec^{-1}}
%\DeclareMathOperator{\vect}{vec}
% use: \ceil*{x}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% new commands
\newcommand*{\mc}[1]{\mathcal{#1}}	% calligraphic font
\newcommand*{\mf}[1]{\mathfrak{#1}}	% fraktur font

\newcommand*{\C}{\mathbb{C}}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\R}{\mathbb{R}}
\newcommand*{\Z}{\mathbb{Z}}

\newcommand{\herm}{{\operatorname{H}}}
\newcommand{\tp}{{\operatorname{T}}}

\newcommand{\dif}{\mathrm{d}}

% comments in text
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{[#1]}}

% align stackrel correctly
\newlength{\leftstackrelawd}
\newlength{\leftstackrelbwd}
\def\leftstackrel#1#2{\settowidth{\leftstackrelawd}%
	{${{}^{#1}}$}\settowidth{\leftstackrelbwd}{$#2$}%
	\addtolength{\leftstackrelawd}{-\leftstackrelbwd}%
	\leavevmode\ifthenelse{\lengthtest{\leftstackrelawd>0pt}}%
	{\kern-.5\leftstackrelawd}{}\mathrel{\mathop{#2}\limits^{#1}}}
\renewcommand{\stackrel}{\leftstackrel}

% bold letters
%	julia code:
%	for i in vcat('A':'Z','a':'z')
%  		println("\\newcommand{\\mb", i, "}{\\bm{", i, "}}")
% 	end
\newcommand{\mbA}{\bm{A}}
\newcommand{\mbB}{\bm{B}}
\newcommand{\mbC}{\bm{C}}
\newcommand{\mbD}{\bm{D}}
\newcommand{\mbE}{\bm{E}}
\newcommand{\mbF}{\bm{F}}
\newcommand{\mbG}{\bm{G}}
\newcommand{\mbH}{\bm{H}}
\newcommand{\mbI}{\bm{I}}
\newcommand{\mbJ}{\bm{J}}
\newcommand{\mbK}{\bm{K}}
\newcommand{\mbL}{\bm{L}}
\newcommand{\mbM}{\bm{M}}
\newcommand{\mbN}{\bm{N}}
\newcommand{\mbO}{\bm{O}}
\newcommand{\mbP}{\bm{P}}
\newcommand{\mbQ}{\bm{Q}}
\newcommand{\mbR}{\bm{R}}
\newcommand{\mbS}{\bm{S}}
\newcommand{\mbT}{\bm{T}}
\newcommand{\mbU}{\bm{U}}
\newcommand{\mbV}{\bm{V}}
\newcommand{\mbW}{\bm{W}}
\newcommand{\mbX}{\bm{X}}
\newcommand{\mbY}{\bm{Y}}
\newcommand{\mbZ}{\bm{Z}}
\newcommand{\mba}{\bm{a}}
\newcommand{\mbb}{\bm{b}}
\newcommand{\mbc}{\bm{c}}
\newcommand{\mbd}{\bm{d}}
\newcommand{\mbe}{\bm{e}}
\newcommand{\mbf}{\bm{f}}
\newcommand{\mbg}{\bm{g}}
\newcommand{\mbh}{\bm{h}}
\newcommand{\mbi}{\bm{i}}
\newcommand{\mbj}{\bm{j}}
\newcommand{\mbk}{\bm{k}}
\newcommand{\mbl}{\bm{l}}
\newcommand{\mbm}{\bm{m}}
\newcommand{\mbn}{\bm{n}}
\newcommand{\mbo}{\bm{o}}
\newcommand{\mbp}{\bm{p}}
\newcommand{\mbq}{\bm{q}}
\newcommand{\mbr}{\bm{r}}
\newcommand{\mbs}{\bm{s}}
\newcommand{\mbt}{\bm{t}}
\newcommand{\mbu}{\bm{u}}
\newcommand{\mbv}{\bm{v}}
\newcommand{\mbw}{\bm{w}}
\newcommand{\mbx}{\bm{x}}
\newcommand{\mby}{\bm{y}}
\newcommand{\mbz}{\bm{z}}

\newcommand{\mbalpha}{{\bm{\alpha}}}
\newcommand{\mbbeta}{{\bm{\beta}}}
\newcommand{\mbgamma}{{\bm{\gamma}}}
\newcommand{\mbdelta}{{\bm{\delta}}}
\newcommand{\mbepsilon}{{\bm{\epsilon}}}
\newcommand{\mbvarepsilon}{{\bm{\varepsilon}}}
\newcommand{\mbzeta}{{\bm{\zeta}}}
\newcommand{\mbeta}{{\bm{\eta}}}
\newcommand{\mbtheta}{{\bm{\theta}}}
\newcommand{\mbiota}{{\bm{\iota}}}

\newtheorem{assumption}{Assumption}
% some phrases:
% ---------------
% due to
% thanks to
% a consequence of ... is
% imply
% yield
% reveal
% observe
% show
% state
% hold
% is true
% can be seen
% by ... we have
% there exists
% there is
% read
% is given by/in
% to this end
% consequently
% summarily
% considering
% with ... in mind
% in view of
% consulting
% hint at
% render
% equality takes place
% predict
% put
% shed light on
% we may estimate
% bears resemblance to
% defer ... to future work
% invoking equation ...
%
%
%
% Transitional Words and Phrases
% ------------------------------
% Illustration
% 
%     Thus, for example, for instance, namely, to illustrate, in other words, in particular, specifically, such as.
% 
% Contrast
% 
%     On the contrary, contrarily, notwithstanding, but, however, nevertheless, in spite of, in contrast, yet,
%     on one hand, on the other hand, rather, or, nor, conversely, at the same time, while this may be true.
% 
% Addition
% 
%     And, in addition to, furthermore, moreover, besides, than, too, also, both-and, another, equally important, first,
%     second, etc., again, further, last, finally, not only-but also, as well as, in the second place, next, likewise,
%     similarly, in fact, as a result, consequently, in the same way, for example, for instance, however, thus, therefore, otherwise.
% 
% Time
% 
%     After, afterward, before, then, once, next, last, at last, at length, first, second, etc., at first, formerly, rarely,
%     usually, another, finally, soon, meanwhile, at the same time, for a minute, hour, day, etc., during the morning, day,
%     week, etc., most important, later, ordinarily, to begin with, afterwards, generally, in order to, subsequently,
%     previously, in the meantime, immediately, eventually, concurrently, simultaneously.
% 
% Space
% 
%     At the left, at the right, in the center, on the side, along the edge, on top, below, beneath, under, around, above,
%     over, straight ahead, at the top, at the bottom, surrounding, opposite, at the rear, at the front, in front of, beside,
%     behind, next to, nearby, in the distance, beyond, in the forefront, in the foreground, within sight, out of sight, across,
%     under, nearer, adjacent, in the background.
% 
% Concession
% 
%     Although, at any rate, at least, still, thought, even though, granted that, while it may be true, in spite of, of course.
% 
% Similarity or Comparison
% 
%     Similarly, likewise, in like fashion, in like manner, analogous to.
% 
% Emphasis
% 
%     Above all, indeed, truly, of course, certainly, surely, in fact, really, in truth, again, besides, also, furthermore, in addition.
% 
% Details
% 
%     Specifically, especially, in particular, to explain, to list, to enumerate, in detail, namely, including.
% 
% Examples
% 
%     For example, for instance, to illustrate, thus, in other words, as an illustration, in particular.
% 
% Consequence or Result
% 
%     So that, with the result that, thus, consequently, hence, accordingly, for this reason, therefore, so, because, since,
%     due to, as a result, in other words, then.
% 
% Summary
% 
%     Therefore, finally, consequently, thus, in short, in conclusion, in brief, as a result, accordingly.
% 
% Suggestion
% 
%     For this purpose, to this end, with this in mind, with this purpose in mind, therefore.
%

